Curricular Object Manipulation in LiDAR-based Object Detection

This paper explores the potential of curriculum learning in LiDAR-based 3D object detection by proposing a curricular object manipulation (COM) framework. The framework embeds the curricular training strategy into both the loss design and the augmentation process. For the loss design, we propose the COMLoss to dynamically predict object-level difficulties and emphasize objects of different difficulties based on training stages. On top of the widely-used augmentation technique called GT-Aug in LiDAR detection tasks, we propose a novel COMAug strategy which first clusters objects in ground-truth database based on well-designed heuristics. Group-level difficulties rather than individual ones are then predicted and updated during training for stable results. Model performance and generalization capabilities can be improved by sampling and augmenting progressively more difficult objects into the training samples. Extensive experiments and ablation studies reveal the superior and generality of the proposed framework. The code is available at https://github.com/ZZY816/COM.

==> contents/1-introduction_zhu.tex <==
\section{Introduction}\label{sec:intro}

\begin{figure}[t]
  \centering
  \begin{subfigure}{0.235\textwidth}
    \includegraphics[trim={22cm 7cm 19cm 0cm},clip, width=\textwidth]{figures/intro1.png}
    \caption{Early stage.}    
      \label{fig:intro1}
    \end{subfigure}
    % \hspace{-1em}
  \begin{subfigure}{0.235\textwidth}
    \includegraphics[trim={21cm 7cm 20cm 0cm},clip, width=\textwidth]{figures/intro4.png}
    \caption{Later stage.}
    \label{fig:intro2}
  \end{subfigure}    
  % \hspace{10pt}
  \caption{
    The proposed Curricular Object Manipulation (COM) works in an easy-to-hard manner.
    In early stages, \textit{COMAug} constrains the augmented objects (highlighted in red) to be easy ones and \textit{COMLoss} down-weights losses from difficulty objects (marked in boxes with thin lines).
    Objects with varying degrees of difficulty are pasted into the point clouds in later stages.
    On the other hand, hard objects will contribute  more to loss values  as training progresses.
    \textbf{Best viewed in color.}
  } \label{fig:intro}
\end{figure}

LiDAR sensors can provide accurate, high-definition 3D measurements of the surrounding environment. Such 3D information play a noninterchangeable role in safety-critical applications like 3D object detection in self-driving. % Aiming to identify objects of interest from the 3D LiDAR point cloud, LiDAR based 3D object detection has advanced significantly.
However, the rich 3D information from LiDAR sensors do not come without problems.
%\footnote{\textcolor{red}{we might need a figure to explain what these data deficiencies are, if short of space maybe in the supplementary?}}.
Usually presented in the form of a point cloud, LiDAR data for object detection suffer from
\begin{enumerate*}[label=(\roman*)]
% \item non-uniformity: the point density decreases monotonically as the laser range increases;
% \item orderless: the geometry of a point cloud remains unchanged even if all of its points are randomly shuffled.
\item point sparsity: as the laser range increases, the point density decreases monotonically.
Meanwhile, due to occlusion and signal miss, the shape of point cloud objects can be extremely incomplete.
Thus, some objects with sparse point cloud are difficult for human annotation, not to mention learning.
\item object sparsity:
Compared with image object detection tasks, sparse point clouds contain
much less input stimuli and positive samples for neural network 
training,
 as depicted in Figure~\ref{fig:intro}.
This problem can hinder the convergence.

 %unlike image tensors, which neighboring pixels/voxels are spatially coherent in the memory layout, depending on the sensor scanning strategies, 3D points may be stored in non-repeatable patterns.
\end{enumerate*}

% To build a robust and performant LiDAR object detector, different data representations have been explored to alleviate the non-uniformity and orderless challenges.
% Feature extraction from the raw orderless point cloud can be made possible by performing radius search or nearest neighbor search in the 3D Euclidean space~\cite{chen2019fast,yang2018ipod,shi2020point,qi2019deep}.
% Another popular solution is to quantize the input point cloud into a fixed grid of voxels~\cite{zhou2018voxelnet} or pillars of voxels~\cite{lang2019pointpillars}. At the price of quantization error, later processing can be done efficiently on the regular voxel pillars or grids~\cite{yan2018second}. 
% Specially, LiDAR scans from mechanical spinning LiDARs can be organized into a compact range image format, which are suitable for adapting 2D image based techniques~\cite{fan2021rangedet,bewley2020range,meyer2019lasernet,chai2021point}.


% \begin{figure}[t]
%   \centering
%     \includegraphics[width=0.55\linewidth]{figures/intro1.png}
%     \caption{\textcolor{red}{Placeholder. Need replacement.} 3D object detection mAP of the car category with moderate difficulties on the KITTI dataset from 2018 to 2020.
%     It is obvious from the figure that the GT-aug strategy boosted the KITTI 3D object detection benchmark by a large margin since its inception~\cite{yan2018second}. GT-Aug has since become the de facto augmentation practice in popular open source toolkits~\cite{mmdet3d2020,openpcdet2020}.}
%     \label{fig:gtaug}
% \end{figure}

% But these different data representations do not change the sparsity of the LiDAR point cloud data.
% Compared with image object detection tasks, sparse point clouds contain much less input stimuli and positive samples for neural network training, as depicted in Figure~\ref{fig:intro}. 
To tackle the issue of object sparsity, 
researchers explore effective data augmentation strategies for faster model convergence and better detection performance~\cite{yan2018second,fang2021lidar,kim2021point,nekrasov2021mix3d,xiao2022polarmix}. 
Among them, GT-Aug~\cite{yan2018second} (see Figure~\ref{fig:gtaug}) is widely adopted. GT-Aug first aggregates ground truth labels from the training dataset into a database. During training, randomly selected samples from the database are inserted into the point cloud to amplify the supervision signal.

% \textcolor{red}{revisit the motivation of COMLoss and COMAug}
Notice that GT-Aug treats all samples in the database equally, and all epochs of the training process equally. 
However, mainly caused by the point sparsity,
the learning difficulties of the samples can vary greatly. 
Moreover,
it has brought to our attention that selecting too many harder examples at early stages may overwhelm the training, while select too many easier samples at the later stages may slow the model convergence. Similar conclusions were also reached independently in the facial recognition field~\cite{huang2020curricularface}. This important finding raises two questions for the widely used GT-Aug strategy: 
\begin{enumerate*}[label=(\roman*)]
\item at a given training stage, how to select samples that benefit the current stage the most,
\item at different training stages, how to adjust the sampling strategies accordingly.
\end{enumerate*}
However, solving these two questions is not yet enough as the source objects in the training point can also be ill-suited for current training.
  Therefore, we raise one additional question as
\begin{enumerate*}[label=(\roman*)]
\item[(iii)] how to properly handle all involved objects can contribute to the model performance.
\end{enumerate*}

\begin{figure}[t]
\centering
\begin{overpic}[width=0.45\textwidth]{figures/intro_gtaug.pdf}
\put(10,9){\makebox[0pt]{\tiny{AVOD\cite{ku2018joint}}}}
\put(30,10){\makebox[0pt]{\tiny{PointRCNN\cite{shi2019pointrcnn}}}}
\put(45,6){\makebox[0pt]{\tiny{F-ConvNet\cite{qi2018frustum}}}}
\put(53,24){\makebox[0pt]{\tiny{\text{STD}\cite{yang2019std}}}}
\put(68,25){\makebox[0pt]{\tiny{\text{PV-RCNN}\cite{shi2020pv}}}}
\put(90,21){\makebox[0pt]{\tiny{\text{Voxel R-CNN}\cite{deng2021voxel}}}}
\put(95,26){\makebox[0pt]{\tiny{\text{PV-RCNN++}\cite{shi2020pv}}}}
\end{overpic}
    \caption{3D object detection mAP of the car category with hard difficulties on the KITTI dataset from 2018 to 2021.
    It is obvious from the figure that the GT-Aug strategy boosts the KITTI 3D object detection benchmark by a large margin since its inception~\cite{yan2018second}. GT-Aug has since become the de facto augmentation practice in popular open source toolkits~\cite{mmdet3d2020,openpcdet2020}.}
    \label{fig:gtaug}
\end{figure}

This work answers the above questions by leveraging curriculum learning.
Curriculum learning draws inspiration from the human cognitive process, which begins with easier concepts and gradually moves on to more complicated ones~\cite{bengio2009curriculum, soviany2022curriculum}.
Enlightened by such easy-to-hard paradigm, we propose a curricular object manipulation (COM) framework for the LiDAR object detection task. Our framework consists of 
\begin{enumerate*}[label=(\roman*)]
\item \textbf{COMLoss} to manipulate the contributions from objects of different difficulties, and
\item \textbf{COMAug} to manipulate the sampling process in GT-Aug.
\end{enumerate*}
%To the best knowledge of the authors, this work is the first to apply curriculum learning to the LiDAR object detection task.

In the COM framework, we employ the classification loss as a simple yet effective proxy for object difficulties.
The COMLoss suppresses loss contributions from hard objects in earlier stages and gradually looses the suppression, as depicted in \cref{fig:intro}.
%To the contrary, modern object detectors often employ hard sample mining in later stages, through focal loss and its variants~\cite{lin2017focal,li2020generalized,zhang2021varifocalnet}.
%Modern object detectors often employ hard sample mining in later stages, through focal loss and its variants~\cite{lin2017focal,li2020generalized,zhang2021varifocalnet}. To the contrary,
%COMLoss suppresses loss contributions from hard objects in earlier stages and gradually looses the suppression, as depicted in \cref{fig:intro}.
Unfortunately, using the classification score as the difficulty proxy for individual objects caused a chicken-and-egg conundrum in COMAug:  
each object must have been sampled recently for augmentation to update its classification score, but without updated classification scores of all objects the sampling process are untrustworthy.
% one object must have been chosen first to calculate its classification score, but given its difficulty estimate it might not be sampled for augmentation.
We design a clustering based method to address such conundrum: objects with similar difficulties are grouped together, and the difficulty estimates are updated for the groups rather than for the individual objects.
During training, hard groups will be sampled with monotonically increasing probabilities as epoch increases, while objects within each group will be sampled uniformly.
In our work, objects are grouped by their geometry attributes, such as distance, dimension, angle, % facade visibility
and occupancy ratio. 

We demonstrate the efficacy of our proposed method through extensive experiments and ablation studies. In summary, our contributions include:
\begin{itemize}
  \itemsep0em
\item We propose the COM framework which embeds the easy-to-hard training strategy into both loss design and augmentation process in LiDAR-based object detection.
  For the loss design, COMLoss is introduced to dynamically predict object-level difficulties, based on which we emphasize objects to different extents when the training proceeds.
  For the augmentation, a well-designed COMAug first clusters objects in ground-truth database with carefully-picked heuristics.
  During training, COMAug updates group-level difficulties and controls augmented objects in a curricular manner.
\item To the best of our knowledge, COM is the first to explore the potentials of curriculum learning in LiDAR-based 3D object detection.
Extensive experiments and ablation studies reveal the superiority and generality of the proposed framework.  
\end{itemize}

% \textcolor{red}{This naive solution should be moved back to later sections.} A naive solution is to initialize object difficulties with a same value and update the sampled objects' difficulties during training.
% However, the probability of one object to be sampled is small (\eg, less than 5\% for class vehicle during one epoch of training in the Waymo Open dataset~\cite{sun2020scalability}) because of the tremendous size of the ground-truth database.
% That makes object difficulties are mostly out-of-date and vulnerable to training noise.

% ----------------------------------------------------------------------------------------------
% Below: Qiang version
% ----------------------------------------------------------------------------------------------
% LiDAR-based 3D object detection, which aims to localize target objects from point clouds, has achieved great advancement in recent years.
% To resolve the irregular and unordered properties of point clouds, a number of successful systems are proposed using different representations including range images~\cite{fan2021rangedet,bewley2020range,meyer2019lasernet}, raw points~\cite{chen2019fast,yang2018ipod,shi2020point,qi2019deep} and voxels/pillars~\cite{zhou2018voxelnet,lang2019pointpillars}.
% Many other works focus on designing more task-suitable network structures/modules such as transformers~\cite{fan2022embracing,sheng2021improving}, sparse convolution~\cite{yan2018second} and range kernel~\cite{chai2021point,fan2021rangedet}.
% Adapting some mature 2D object detection frameworks into the task is also a popular direction~\cite{yin2021center,deng2021voxel}.
% Besides, the sparsity of point clouds is another issue where most regions of 3D space only contain backgrounds or are even without measurements as depicted in \cref{fig:intro}.
% % The issue can cause severe imbalance between foregrounds (marked in blue in \cref{fig:intro}) and backgrounds and that motivates a line of data augmentation methods~\cite{yan2018second,fang2021lidar,kim2021point,nekrasov2021mix3d,xiao2022polarmix,chen2020pointmixup,hahner2020quantifying,li2020pointaugment,sheshappanavar2021patchaugment}.
% This issue motivates a line of data augmentation methods~\cite{yan2018second,fang2021lidar,kim2021point,nekrasov2021mix3d,xiao2022polarmix}.
% Among them, \textit{GT-Aug}~\cite{yan2018second} is a popular one which has been widely used in current literature~\cite{yan2018second,yang2022graph,yang20203dssd,yin2021center,shi2020pv,shi2021pv} and projects (\eg, OpenMMLab~\cite{mmdet3d2020} and OpenPCD~\cite{openpcdet2020}).
% \textit{GT-Aug} first generates a ground-truth database by collecting labels of target objects from training dataset.
% Fast convergence and better performance can be achieved by inserting sampled instances (marked in red in \cref{fig:intro}) into current training point.
% 
% Despite of great progress in representations, networks and data augmentations, very limited efforts are paid into training strategies in LiDAR-based 3D object detection.
% Prior methods usually treat all target objects equally in the whole training process.
% In addition, \textit{GT-Aug} randomly selects objects from the database and is unknown if these instances can benefit current training.
% The egalitarianism may lead to convergence issue at the early stage where semi-hard/hard samples overwhelms the training, and may make semi-hard/hard samples not fully exploited at later stages~\cite{huang2020curricularface}.
% These issues raise two questions:
% (1) which objects to be emphasized and how to emphasize them in different stages, and (2) which objects to be selected from the database can accord most to current model training.
% 
% 
% This work attempts to resolve two questions by exploring potentials of curriculum learning in the unexplored LiDAR-based 3D object detection.
% Curriculum learning (CL) draws inspiration from human cognitive process, which begins with learning easier concepts and then gradually processes to learning more complicated concepts~\cite{bengio2009curriculum, soviany2022curriculum}.
% % The straightforward yet efficacy paradigm feeds the model with progressively more difficult samples in order to improve model performance and generalization.
% Following the high-level idea of easy-to-hard training, we propose a framework called curricular object manipulation (COM), which consists {\bf (a)} COMLoss to manipulate the losses from objects of different difficulties and {\bf (b)} COMAug to manipulate the object sampling process in \textit{GT-Aug}.
% During training, COMLoss suppresses losses from hard objects in early stages while looses the suppression as shown in \cref{fig:intro}.
% The strategy works better than the conventional schemes of emphasizing (semi-)hard samples in later stages, which may be unnecessary as object detectors are usually built-in with hard-mining scheme with losses such as focal loss~\cite{lin2017focal} and its variations~\cite{zhang2021varifocalnet,li2020generalized}.
% To determine object difficulty, we follow the idea that loss value is an alternative indicator~\cite{kong2021adaptive,huang2020curricularface,meng2021magface,ren2018learning} and employ the losses from the classification branch.
% We find the criterion is simple yet efficient and reserve using intricate criteria~\cite{saxena2019data,castells2020superloss} for future works.
% 
% 
% In accordance with the design of COMLoss, COMAug also estimate object difficulty by the classification loss if an object is augmented into one training point.
% One problem here is that the existence of object difficulties is the prerequisite of the difficulty-adaptive sampling in COMAug, but difficulty of one object can only be updated if it's sampled for augmentation.
% A naive solution is to initialize object difficulties with a same value and update the sampled objects' difficulties during training.
% However, the probability of one object to be sampled is small (\eg, less than 5\% for class vehicle during one epoch of training in in waymo~\cite{sun2020scalability}) because of the tremendous size of the ground-truth database.
% That makes object difficulties are mostly out-of-date and vulnerable to training noise.
% To cope with these issues, we design a clustering method which groups objects with similar difficulties and update the group difficulty scores rather than the individual scores.
% % In this way, the group difficulties can be updated frequently and are reluctant to noise.
% Thanks to the rich physical properties, more potential grouping strategies can be employed for point clouds than those for conventional camera images.
% In our work, we cluster objects using attributes including distance, size, facade and occupancy ratio.
% During training, we design an epoch-adaptive curve which assigns hard groups with progressively increasing probabilities to be sampled, and randomly pick objects for augmentation inside a sampled group.
% This efficacy of the COM framework is further proved by our experiments and ablation studies.
% To sum up, our major contributions are as follows:
% \begin{itemize}
%   \itemsep0em
% \item For the first time, COM explores the potentials of curriculum learning in LiDAR-based 3D object detection.
%   The framework embeds the easy-to-hard training strategy into both loss design and augmentation process.
% \item We propose COMLoss to dynamically predict object-level difficulties, based on which we emphasize objects to different extents when the training proceeds.
% \item We propose the COMAug to cluster objects in ground-truth database with well-designed heuristics.
%   During training, COMAug updates group-level difficulties and controls the augmented objects in a curricular manner.
% \item Extensive experiments and ablation studies reveal the superior and generality of the proposed framework.
% \end{itemize}


% ----------------------------------------------------------------------------------------------
% Below: very initial version
% ----------------------------------------------------------------------------------------------

% Curriculum Learning (CL) draws inspiration from human cognitive process, which begins with learning easier concepts and then gradually processes to learning more complicated concepts~\cite{bengio2009curriculum, soviany2022curriculum}.
% The straightforward yet efficacy paradigm feeds the model with progressively more difficult samples in order to improve model performance and generalization.
% Two crucial components contribute to the curricular training progress:
% 1) the pacing function to arrange the learning process and
% 2) the difficulty criterion to measure the difficulty level of each sample.
% Single step pacing, fixed exponential pacing and varied exponential pacing are the common choices of the pacing function~\cite{hacohen2019power,kong2021adaptive}.
% Some other strategies such as consistently suppressing hard samples~\cite{castells2020superloss} can be useful in particular scenarios.
% For the difficulty criterion, heuristic knowledge~\cite{soviany2021curriculum} or pre-trained models~\cite{ren2018learning,lu2022pcc} can be utilized to determinate sample difficulties.
% To better accord with the learning procedure, a growing line of literature~\cite{saxena2019data,castells2020superloss,kong2021adaptive,chang2017active} resorts to dynamically criterion by predicting difficulties with some learnable parameters and makes some impressive progresses.


% Despite of the great breakthrough of curriculum learning, current literature still overwhelmingly specializes on the classification task~\cite{hacohen2019power,ren2018learning,jiang2018mentornet,chang2017active,kong2021adaptive,lu2022pcc,kong2021adaptive} and overlooks object detection~\cite{saxena2019data,castells2020superloss}, let alone the LiDAR-based detection.
% There are two potential causes of the situation.
% Firstly, the conventional curriculum learning treats one sample as the entirety and performs sample-wise manipulation during training.
% However, one sample in object detection typically contains objects of varying difficulties, necessitating object-level difficulty predictions and pacing patterns.
% Secondly, the object detection community favors the hard-mining strategy, which has been amply validated by a great proportion of related works (\eg, OHEM~\cite{shrivastava2016training}, focal loss~\cite{lin2017focal} and its variations~\cite{zhang2021varifocalnet,li2020generalized}).
% In SuperLoss~\cite{castells2020superloss}, curriculum learning performs well on noisy datasets but makes no difference with baseline object detector with normal training.
% Extra efforts are required to fit the easy-to-hard scheme on the detection task.


% This work explores potentials of curriculum learning in an unexplored area called LiDAR-based 3D object detection.
% In the proposed curricular object manipulation (COM) framework, we design a curricular loss termed COMLoss to address the two aforementioned general challenges.
% Following the idea that loss value is an alternative indicator of difficulty~\cite{kong2021adaptive,huang2020curricularface,meng2021magface,ren2018learning}, we collect the losses of each object in the classification branch and take the max value as the object difficulty.
% Compared to the fixed criterion using heuristic knowledge~\cite{soviany2021curriculum} or pre-trained models~\cite{ren2018learning,lu2022pcc}, the loss-based difficulty criterion can accord better with current model status.
% Additionally, the strategy requires no extra computations and is simple to implement.
% We reserve the use of more intricate criteria~\cite{saxena2019data,castells2020superloss} for future works.
% For the pacing function, we found that the easy-to-hard scheme also works for the task but need a few modifications.
% To be more specific, object detectors usually uses hard-mining strategies with losses such as focal loss~\cite{lin2017focal} and its variations~\cite{zhang2021varifocalnet,li2020generalized}.
% Emphasizing hard samples in later stages is no longer that necessary in this situation.
% Instead, we propose to suppress losses from difficult samples in the early stages (\cref{fig:intro1}) and loose the suppression with training progresses (\cref{fig:intro2}).
% In our experiments, we find that the modified curricular scheme performs better than the conventional easy-to-hard scheme.


% Curriculum Learning (CL) draws inspiration from human cognitive process, which begins with learning easier concepts and then gradually processes to learning more complicated concepts~\cite{bengio2009curriculum, soviany2022curriculum}.
% The straightforward yet efficacy paradigm feeds the model with progressively more difficult samples in order to improve model performance and generalization.
% Two crucial components contribute to the curricular training progress:
% 1) the pacing function to arrange the learning process and
% 2) the difficulty criterion to measure the difficulty level of each sample.
% Single step pacing, fixed exponential pacing and varied exponential pacing are the common choices of the pacing function~\cite{hacohen2019power,kong2021adaptive}.
% Some other strategies such as consistently suppressing hard samples~\cite{castells2020superloss} can be useful in particular scenarios.
% For the difficulty criterion, heuristic knowledge~\cite{soviany2021curriculum} or pre-trained models~\cite{ren2018learning,lu2022pcc} can be utilized to determinate sample difficulties.
% To better accord with the learning procedure, a growing line of literature~\cite{saxena2019data,castells2020superloss,kong2021adaptive,chang2017active} resorts to dynamically criterion by predicting difficulties with some learnable parameters and makes some impressive progresses.


% Despite of the great breakthrough of curriculum learning, current literature still overwhelmingly specializes on the classification task~\cite{hacohen2019power,ren2018learning,jiang2018mentornet,chang2017active,kong2021adaptive,lu2022pcc,kong2021adaptive} and overlooks object detection~\cite{saxena2019data,castells2020superloss}, let alone the LiDAR-based detection.
% There are two potential causes of the situation.
% Firstly, the conventional curriculum learning treats one sample as the entirety and performs sample-wise manipulation during training.
% However, one sample in object detection typically contains objects of varying difficulties, necessitating object-level difficulty predictions and pacing patterns.
% Secondly, the object detection community favors the hard-mining strategy, which has been amply validated by a great proportion of related works (\eg, OHEM~\cite{shrivastava2016training}, focal loss~\cite{lin2017focal} and its variations~\cite{zhang2021varifocalnet,li2020generalized}).
% In SuperLoss~\cite{castells2020superloss}, curriculum learning performs well on noisy datasets but makes no difference with baseline object detector with normal training.
% Extra efforts are required to fit the easy-to-hard scheme on the detection task.

% This work explores potentials of curriculum learning in an unexplored area called LiDAR-based 3D object detection.
% In the proposed curricular object manipulation (COM) framework, we design a curricular loss termed COMLoss to address the two aforementioned general challenges.
% Following the idea that loss value is an alternative indicator of difficulty~\cite{kong2021adaptive,huang2020curricularface,meng2021magface,ren2018learning}, we collect the losses of each object in the classification branch and take the max value as the object difficulty.
% Compared to the fixed criterion using heuristic knowledge~\cite{soviany2021curriculum} or pre-trained models~\cite{ren2018learning,lu2022pcc}, the loss-based difficulty criterion can accord better with current model status.
% Additionally, the strategy requires no extra computations and is simple to implement.
% We reserve the use of more intricate criteria~\cite{saxena2019data,castells2020superloss} for future works.
% For the pacing function, we found that the easy-to-hard scheme also works for the task but need a few modifications.
% To be more specific, object detectors usually uses hard-mining strategies with losses such as focal loss~\cite{lin2017focal} and its variations~\cite{zhang2021varifocalnet,li2020generalized}.
% Emphasizing hard samples in later stages is no longer that necessary in this situation.
% Instead, we propose to suppress losses from difficult samples in the early stages (\cref{fig:intro1}) and loose the suppression with training progresses (\cref{fig:intro2}).
% In our experiments, we find that the modified curricular scheme performs better than the conventional easy-to-hard scheme.


% Apart from the two aforementioned challenges, there is a noteworthy term called \textit{GT-Aug} for LiDAR-based 3D object detection.
% As indicated in \cref{fig:intro}, point clouds are usually captured from a wide physical range while target objects (marked in blue) are of small size and sparse distribution.
% The imbalance issue between foregrounds and backgrounds are more serious that that of image-based object detection.
% To relieve the issue, Second~\cite{yan2018second} proposes the \textit{GT-Aug} which first generates a ground-truth database  by collecting labels of all target objects from training dataset.
% During training, several ground truths are randomly sampled from the database and concatenated into current training point.
% The simple strategy leads to fast convergence and better performance, and  has been widely used in current literature~\cite{yan2018second,yang2022graph,yang20203dssd,yin2021center,shi2020pv,shi2021pv} and popular projects (\eg, OpenMMLab~\cite{mmdet3d2020} and OpenPCD~\cite{openpcdet2020}).
% We argue that randomly sampling ground-truth database in all training stages can be optimized by a curricular way as shown in \cref{fig:intro}.
% In accordance with the design of COMLoss, we also estimate the difficulty of a object in the database by its classification loss if it's augmented to one training point.
% However, the curricular augmentation relies on pre-calculated difficulties of all objects in the ground-truth database.
% For example, we should know in advance which objects are easy if we want to select some easy objects to augment in early stage.
% The naive solution is to initialize all objects with the same difficulty score and update them if they are sampled during augmentation.
% This solution however has two significant flaws:
% Considering the large volume of the ground-truth database, this solution has two flaws: 
% (1) The average number of one object to be sampled in the whole training process is small.
% For example, in our experiments, the number is less than 1 for the waymo\qtext{calculate the number and cite the waymo} database which contains over 2 million objects.
% Therefore, object difficulties are mostly not updated or predicted by out-of-date models.
% (2) The limited calculation numbers can introduce training noisy to the predictions and that also makes the difficulty score unreliable.
% Therefore,  we design a clustering method which groups objects with similar difficulties in the database and update the group difficulty scores rather than the individual scores.
% In this way, the group difficulties can be updated frequently and are reluctant to noise.
% Thanks to the rich physical properties, point cloud data contains more possible grouping strategies than conventional camera images.
% In our work, we cluster objects by their attributes including distance, size, facade and occupancy ratio for clustering.
% During training, we first select groups based on their difficulties and then randomly sample objects in the group for augmentation.
% We name the augmentation process as COMAug and prove its superior by our experiments.
% To sum up, our major contributions are as follows:
% \begin{itemize}
%   \itemsep0em
% \item For the first time, COM explores the potentials of curriculum learning in LiDAR-based 3D object detection.
%   The framework embeds the easy-to-hard training strategy into both loss design and augmentation process.
% \item We propose the COMLoss which dynamically predicts object-level difficulty scores and emphasizes objects of different scores based on training stages.
% \item We propose the COMAug which clusters objects in ground-truth database based on well-designed heuristics.
%   During training, COMAug updates group-level difficulties and controls the augmented objects in a curricular way.
% \item Extensive experiments and ablation studies reveal the superior and generality of the proposed framework.
% \end{itemize}

